Uni6Dv2: Noise Elimination for 6D Pose Estimation

Uni6D is the first 6D pose estimation approach to employ a unified backbone network to extract features from both RGB and depth images. We discover that the principal reasons of Uni6D performance limitations are Instance-Outside and Instance-Inside noise. Uni6D's simple pipeline design inherently introduces Instance-Outside noise from background pixels in the receptive field, while ignoring Instance-Inside noise in the input depth data. In this paper, we propose a two-step denoising approach for dealing with the aforementioned noise in Uni6D. To reduce noise from non-instance regions, an instance segmentation network is utilized in the first step to crop and mask the instance. A lightweight depth denoising module is proposed in the second step to calibrate the depth feature before feeding it into the pose regression network. Extensive experiments show that our Uni6Dv2 reliably and robustly eliminates noise, outperforming Uni6D without sacrificing too much inference efficiency. It also reduces the need for annotated real data that requires costly labeling.

==> sec/1intro_old.tex <==
\section{INTRODUCTION}
\label{Introduction}

\begin{figure}[htbp]
\vspace{.3in}
	\centering
	\subfigure[]{\includegraphics[width=0.85\linewidth]{figures/fig1a.png}%
	    \label{fig:fig1_outside}
		}
	\subfigure[]{\includegraphics[width=0.85\linewidth]{figures/fig1b.png}%
	    \label{fig:fig1_inside}
		}\\\vspace{-0.4cm}
	\subfigure[]{\includegraphics[width=0.95\linewidth]{figures/fig1c.png}%
	    \label{fig:fig1_1}
		}
	\subfigure[]{\includegraphics[width=0.85\linewidth]{figures/fig1d.png}%
		\label{fig:fig1_2}}

    \caption{Illustration of noise problem in 6D pose estimation.
     (a) Examples of instance-outside noise, which comes from background pixels outside the target instances. 
     (b) Examples of instance-inside noise, which comes from the unreliable depth data.
     (c) Quantitative results of instance-inside noise according to the depth reprojection error statistics. 
     (d) Uni6D results under various real data percentages and noise elimination methods.
     Eliminating the noise improves performance and reduces the need for real data in training set.
     }
	\label{fig:hor_2figs_1cap}
\end{figure}

6D pose estimation is essential for emerging applications such as intelligent robotic grasping\Citep{collet2011moped,tremblay2018deep}, autonomous driving\Citep{geiger2012we,xu2018pointfusion,chen2017multi}, and augmented reality\Citep{marchand2015pose}.
%
The primary goal of 6D pose estimation is to determine the 6D pose of an object, which includes its location and orientation.
%
The RGB-D sensor can augment the conventional RGB image with depth information in a per-pixel basis and provide directly geometry information, making it a more appealing data source for 6D pose estimation as it becomes more feasible and affordable.
%
The only fly in the ointment is that it inevitably introduces physical noise when acquiring depth information\Citep{zhang2012microsoft, mallick2014characterizations,zhang2018deep, sweeney2019supervised, ji2021calibrated}.

Considering the heterogeneity of RGB data and depth data, previous state-of-the-art methods\Citep{densefusion,pvn3d,ffb6d} typically handle them with two backbone networks separately, in which, 2D CNN is used for RGB data and PointNet\Citep{pointnet} or PointNet++\Citep{pointnet++} for depth data.
%
Recently, a new approach called Uni6D\Citep{uni6d} subverts the above practice by adding extra UV information, i.e., coordinates of each pixel, into the RGB-D input to solve the "projection breakdown"\Citep{uni6d} issue.
It leverages basic framework of Mask R-CNN\citep{maskrcnn}, including RPN, RoI Align, and especially the unified CNN backbone to extract features from RGB and depth images possible, resulting in an efficient and straightforward realization pipeline.
%
However, Uni6D ignores the potential pitfalls hidden in its straightforward pipeline and the input depth data, severely limiting its performance.
%



% may need a figure to directly show the noise
We find that the main sources of Uni6D's potential pitfalls are two types of noise: instance-outside noise introduced by the RoI-based 6D pose estimation methodology, and instance-inside noise from the unreliable depth data.
%
As shown in Fig.~\ref{fig:fig1_outside}, the instance-outside noise comes from the background pixels outside the target instances, and Uni6D introduced it in the pose regression with its detection and pose regression pipeline. Since the deep features of CNN have corresponding receptive fields, the information out of the instance will also be included in the RoI features obtained by the RPN and RoI Align. Because the feature outside the instance isn't useful for pose estimation, this background information can even interference the pose regression. For the instance-inside noise, it is introduced by depth sensor during capturing depth information, as exampled in Fig.~\ref{fig:fig1_inside}.

To quantify the above noise and their impact, we construct several corresponding experiments. As shown in Fig.~\ref{fig:fig1_1}, we provide the statistic of instance-inside noise of the YCB-Video\Citep{posecnn} dataset by calculating the depth deviation according to depth reprojection error, which indicates that there is depth noise in the dataset. Then, we investigate the effects of performance by removing these kinds of noise incrementally in Fig.~\ref{fig:fig1_2}. We use the ground truth bounding box and mask to crop and mask the RoI of each instance to filter out instance-outside noise. We use the depth calculated by reprojection as the ground truth to remove instance-inside noise.
%
We can observe that removing these two types of noise gradually can significantly improve the accuracy on the YCB-Video dataset, and reduce the need for real data to train the model.
%
According to above experimental results, we believe that each kind of noise will affect the performance of the model. Worse still, limited by the high cost of annotation, existing datasets such as YCB-Video\Citep{posecnn} and LineMOD\Citep{hinterstoisser2011multimodal} include a lot of synthetic data without depth noise in training set and put the real data with depth noise in test set. This train-test gap as shown in Fig.~\ref{fig:fig1_1} further amplifies the negative effect of depth noise. 

%The parallel tasks of detection, segmentation and 6D pose regression in Uni6D depend on the different size of the receptive field, namley detection and %segmentation need the larger receptive field, which introduces information out of targets and become a kind of noise for 6D pose regression. Moreover, %the extra UV information may be regared as noise for detection and segmentation, which breaks the translation invariance of convolution.
%
To this end, we propose Uni6Dv2, a two-step denoising 6D pose estimation method based on the simple yet effective design. 
%
%Uni6Dv2 improves performance without sacrificing inference efficiency by leveraging different strategies to mitigate different noise while %maintaining the unified backbone for RGB and depth data paradigm.
%
% Considering that the parallel tasks of detection, segmentation and 6D pose regression in Uni6D depend on the different size of the receptive field, we take a independent detection and segmentation task, namely detection and segmentation need the larger receptive fields, which introduces irrelevant non-instance information and become a kind of noise for 6D pose regression. Moreover, the extra UV information may be regared as noise for detection and segmentation, which breaks the translation invariance of convolution.
%
The first step aims to address the instance-outside noise, and Uni6Dv2 predicts the instance segmentation mask of each instance from the RGB-D image to filter out irrelevant non-instance pixels. 
%
In the second step, a depth denoising module is used to correct the depth feature with corresponding depth normal and XY before feeding them into the subsequent pose regression network.
%
% This simple modification has been proved effective in balancing speed and accuracy on the YCB-Video and LineMOD datasets. 

The main contributions of this work are:
1) we uncover different potential noise that severely limit the performance of RoI-based 6D pose estimation methods, and categorize them as instance-outside noise and instance-inside noise;
2) we propose a two-step denoising pipeline to address the noise problem in the original Uni6D, which uses the instance segmentation network to filter out the instance-outside noise in the first step and a depth denoising module to handle instance-inside noise in the second step; 
3) our approach advances state-of-the-art by 0.2$\%$ on the AUC  ADD-S metric and achieves 91.5$\%$ on the AUC ADD(S) metric for YCB-Video dataset. In particular, the performance outperforms Uni6D by a large margin, especially in scenes with insufficient real data.

% \begin{enumerate}

% \item We uncover a variety of noise that severely limit the performance of RoI-based 6D pose estimation methods, and categorize them as instance-outside noise and instance-inside noise.

% \item We propose a two-step framework to address the noise problem in the original Uni6D, which uses the instance segmentation network to filter the instance-outside noise in the first step and a depth denoise module to correct instance-inside noise in the second step.

% \item Our approach advances state-of-the-art by 0.2$\%$ on the ADD-S metric and achieves 91.5$\%$ on the ADD(S) metric for YCB-Video dataset. In particular, the performance outperforms Uni6D by a wide margin, especially in scenes with insufficient real data.

% \end{enumerate}

% Recent advances in RGB-D based 6D pose estimation \cite{densefusion, pvn3d, ffb6d} extracts the appearance feature and geometry information by two different backbone networks separately, namely the 2D CNN for RGB images and per pixel PointNet\cite{pointnet} or PointNet++\cite{pointnet++} for depth data. 
% %
% After that, the learned features would be fed into a fusion module. 
% %
% However, the complicated process of the above methods brings great difficulties in industry applications.
% %
% To simplify the pipeline, Uni6D\cite{uni6d} used a unified backbone to extract features from RGB-D images, which achieved the balance of speed and accuracy. 
% %
% However, there is still a gap between the performance of Uni6D and the keypoint-based method\cite{pvn3d,ffb6d}, and the gap is greater in the LineMOD data set through insufficient real training data. 
% %
% The main reason for that is the Uni6D did not consider the noise from the background pixels and unreliable raw depth.
% %
% Because of the existence of noise, the gap is larger generally.
% %
% In addition, other methods\cite{pvn3d,ffb6d} leverage the voting mechanism to weaken the noise pixels with fewer votes, and the clustering method is introduced to further strengthen the clustering center, which can be regarded as a denoising strategy for obtaining high-quality depth cues. 
% %
% However, these key points rely on extra post-processing to estimate the 6D pose.

% Uni6D is an RoI-based instance level 6D pose estimation method, using RoI features to regress the rotation and translation directly.
% %
% Such a simple design greatly reduces the computational cost, but there is no attempt was made to denoise.
% %
% Consequently, this paper first analyzes the source of the noise, then we use different strategies to mitigate different noise so as to achieve a balance between speed and accuracy. 
% %
% The noise of Uni6D mainly comes from three aspects: the region out of interest, the background of RoI( Region of Interest), and the inaccurate raw depth. 
% %
% The first two noise are both about the pixels out of the target objects, which are usually fused by convolution operations, and are invalid for objects to be estimated. 
% %
% The last kind of noise is the error from depth caused by the depth sensor, and the misleading depth breaks the 3D projection equation directly.
% %
% We also calculate the depth error according to reprojected depth on the YCB data set.
% %
% Moreover, we provide variance of errors to measure the fluctuation of depth deviation.
% %
% The larger the variance is, the more difficult it is for the model to learn the fixed deviation of depth.

% In order to verify the promotion that removing these three kinds of noise, we eliminate denoise in turn, and the AUC of ADDS-0.1 on the YCB-Video \cite{posecnn} dataset is shown in Fig. 1a, which reveals that there has been a gradual drop during the noise elimination. 
% %
% Additionally, the impact of denoising during the realistic training data is insufficient can be clearly seen in Fig. 1b, the accuracy of denoising falls slightly, which outperforms uni6D.
% %
% Extensive experiments also show that the performance of the 6D pose is gradually improved with the removal of noise, which indicates that our idea of denoising based on Uni6D is correct. 
% %
% In this work, we propose a two-step network. 
% %
% The first step consists of object detection and instance segmentation, which inherit the legacy of the Mask R-CNN\cite{maskrcnn}.
% %
% The second step is to obtain 6D pose regression results, using the patches cropped by the detection bounding box from the first step as input.
% %
% Specifically, before those patches are fed into the second step, we use the segmentation mask obtained from the first step to filter the noise from the background. 
% %
% Moreover, the depth denoise module is inserted before the RT head, which corrects the depth, depth normal, and XY.
% %
% We evaluate the proposed method on the YCB-Video and LineMOD datasets and demonstrate its performance by taking into account the trade-off between speed and accuracy. 
% %
% In particular, the ablation study on the YCB-Video dataset illustrates the effectiveness of denoising.

% To summarize, the main contributions of this work are as follows: 
% %
% First, we uncover that noise has a significant interference on the 6D pose estimation for uni6D, especially in the case of insufficient real training data, and that is common in practical applications.
% %
% We further categorize the noise into three types, which are region out of interest, background pixel in the RoI, and depth error.
% %
% Finally, we propose a two-step method uni6Dv2 with a depth denoise module to alleviate the aforementioned noise, which outperforms Uni6D by a large margin and becomes state-of-the-art. 
% %
% The inference speed is slower than Uni6D slightly, but our method speeds up the inference compared to the keypoint-based methods, which balances the speed and accuracy well.
 


==> sec/3approach_bk.tex <==
\section{APPROACH}
% 第一段：章节分布介绍
% 3.1：review uni6D
%    是否需要PRJ公式？还是说重新浓缩一个公式表示整个uni6D，类似pointnet++
% 3.2：overall pipeline (two step)
%       3.2.1 subsubsection: first step 
%       3.2.2 subsubsection: second step
% 
\label{headings}
Our work can be viewed as an extension of Uni6D\Citep{uni6d} with a novel two-step denoising pipeline. We first review Uni6D (Sec.~\ref{sec:review_uni6d}), and then give the details of the proposed method, including the denoising processes of instance-outside noise and instance-inside noise (Sec.~\ref{sec:method}). Finally, the details of loss function are provided (Sec.~\ref{sec:loss}).
% We find that the noise has a significant interference on 6D pose estimation, thus we focus mainly on denoising while maintaining time efficiency. Our framework inherits the concise design of uni6D \Citep{uni6d}, with added denoise structure. We first review uniu6D and  present a comprehensive denoise pipeline. Then, introduce the details of instance-outside noise elimination. Finally, we propose our depth denoise module that is able to calibrate depth, XY, and depth normal from instance-inside noise.

\subsection{Review of Uni6D: a Unified CNN Framework for 6D Pose Estimation}
\label{sec:review_uni6d}
% Most previous approaches use two heterogeneous networks to extract the feature of RGB and depth images separately. Uni6D subverted the above practice and use an unified network by adding extra UV information to input data. 
%Uni6D fixed the "projection breakdown" issue caused by the CNN operation and spatial transformations by adding extra UV information (Plain UV, XY, PE) with NRM together to RGB-D images, allowing for simultaneous feature extraction of RGB and depth data with an unified network. 
Uni6D addressed the "projection breakdown" problem, which arises from the CNN and spatial transformations, by adding extra visible point coordinates in both the image plane and 3D space (Plain UV, XY) with depth normal(NRM) into RGB-D images. This enables simultaneous feature extraction of RGB and depth data using a unified network. 
% Given the input RGB and depth data, Uni6D defines a function $f$ that maps the feature of RoIs and corresponding UV information to a pose vector:
% \begin{equation}
%     \begin{split}
%         & UV = \{Plain UV, XY, PE\} \\
%         & Pose = f(RoI Align(RGB, Depth, NRM, UV))
%     \end{split}
% \end{equation}
It took the Mask R-CNN structure and extended it with an extra RT head for estimating rotation and translation parameters, and an abc head regressing visible points $(a,b,c)$ from the CAD model to directly estimate the 6D pose. It achieved impressive results on existing 6D pose estimation benchmarks. However, it suffered from instance-outside noise caused by background pixels and ignored instance-inside noise in the input depth data. In the following section, we will present our two-step denoising method to tackle these challenges.

% The essential reason for that is CNN and some spatial transformations such as crop, RoI-Align \Citep{maskrcnn}, pooling transform visible point's 2D pixel coordinate (UV), which break the physical relation between pixel value and UV, eventually lead to the projection breakdown. The classic 3D vision projection equation is 
% \begin{equation} \label{equ:prj}
%   \begin{bmatrix}
%     u \\
%     v \\
%     1 
%   \end{bmatrix}
%     =
%     \frac{K}{d}
%   \begin{bmatrix}
%     x \\
%     y \\
%     d 
%   \end{bmatrix}
%     =
%   \frac{K}{R_z(a,b,c)+T_z}
%     \begin{pmatrix} 
%     R\times \begin{bmatrix}
%     a \\
%     b \\
%     c
%   \end{bmatrix} + T\end{pmatrix},
% \end{equation}
%  To solve this problem, uni6D concatenated UV with the RGB-D data along the channel dimension which unify the backbone for RGB and depth. The framwork inherited the structure of Mask R-CNN\cite{maskrcnn} with an extra RT head and abc head to estimate the 6D pose directly.It achieved the balance of speed and accuracy. However, it is still lower than the state-of-the-art methods, and lacking the ability to filter the noise is the key reason. It is worth emphasizing that the accuracy gap is greater under insufficient real data scenes. We will introduce our two-step framework in the next section to resolve the limitation.

\begin{figure*}[t]

    \centering
    \includegraphics[width=0.8\textwidth]{figures/fig2.png}

    \caption{Architecture overview of Uni6Dv2. Uni6Dv2 consists of two denoising steps: the first step removes instance-outside noise by adopting the Mask R-CNN to crop and mask the information about the instance, while the second step removes the instance-inside noise by utilizing a depth denoising module and a depth information estimation auxiliary task to calibrate the depth feature before the 6D pose regression. The auxiliary supervision labels $D^{'}$, $XY^{'}$ and $NRM^{'}$ are calculated by projecting the CAD model with the rotation and translation ground truth.}
    \label{fig:framework}
\end{figure*}

\subsection{Comprehensive Denoising Pipeline}
\label{sec:method}
To effectively suppress the instance-outside and instance-inside noise, we propose a novel two-step denoising pipeline named Uni6Dv2, which is illustrated in Fig.~\ref{fig:framework}. Our method is based on Uni6D's basic methodology, which involves adding various UV information to input RGB-D data and regressing 6D pose directly. The instance-outside noise is handled in the first denoising step. For an input RGB-D image, we perform instance segmentation with Mask R-CNN to filter out the instance-outside pixels in RGB, depth, Plain UV, XY, NRM and corresponding position encoding(PE). The above data is then fed into the second step. A depth denoising module and a depth reconstruction task are proposed in the second denoising step to calibrate the feature extracted from the data output by the first step, making it easier for subsequent networks to regress more accurate 6D pose. We use Uni6D's RT head to regress the 6D pose directly, while regressing corresponding coordinates in CAD model by abc head as the auxiliary training branch.


% Our method follows the basic methodology in Uni6D that adding various UV information into input RGB-D data and directly regresses 6D pose. In order to avoid repeating the mistakes of introducing background noise in the feature extraction of RoI in Uni6D, our method takes an image-level instance data extraction, rather than the previous feature-level. Specially, the first denoising step is used to remove the instance-outside noise, which adopts Mask R-CNN to obtain the box and mask so as to crop the instance from the RGB-D image and remove the non-instance part. It is worth emphasizing that the corresponding input includes plain UV, XY, NRM will also be cropped and masked. In the next step, we extract the feature of the above data from the first step through ResNet, then feed it into the proposed depth denoising module to calibrate the depth to filter the instance-inside noise. 
% Our depth denoising module takes the feature of the data from the first step, and outputs features contains the calibrated depth information, making it easier for subsequent models to regress more accurate 6D pose.

% The calculation process can be summarized as:
% \begin{equation}
%     \begin{split}
%         & UV = \{Plain UV, XY, PE\} \\
%         & RGB_{i}, Depth_{i}, NRM_{i}, UV_{i} = RoI Align(RGB, Depth, NRM, UV) \\
%         & F = Backbone(RGB_{i}, Depth_{i}, NRM_{i}, UV_{i}) \\
%         & Pose = f(d(F))
%     \end{split}
% \end{equation}
% Given input RGB pixels $\{x_1,x_2,...,x_n\}$, we use instance segmentation method to choose a subset of pixels $\{x_{i_1},x_{i_2},...,x_{i_m}\}$, such that $x_{i_j}$ is the visible point of target object. And the corresponding UV set is $\{y_{i_1},y_{i_2},...,y_{i_m}\}$.
%
% In the second step, we use unified backbone $f$ to extract RGB and UV features  simultaneously, then 


% \subsection{Instance-outside Noise Elimination}

% Mask is a common choise for instance-outside noise elimination, and most of the previous methods adopt the mask at the feature level, without too much consideration of the position. However, the location of the mask is related to the degree of denoising because the irrelevant information of the receptive field will be continuously fused by CNN. Therefore, To obtain the input-based mask, we saperate detection and segmentation from uni6D. In addition, we also find that dependence of UV encoding is discrepant between detection and 6 DoF pose estimation, UV encoding breaks the convolution translation invariance, which is not friendly to the detection and segmentation, especially when the amount of data is insufficient.


% \subsection{Instance-inside Noise Elimination}
% A given depth image contains two parts of the error, the numerical error about depth estimation and the complete dropouts of some pixels, and both two errors lead to the breakdown of the projection. For the dropouts, uni6D take a classical image processing algorithm\cite{ku2018defense} to fill holes of the raw depth before regressing the 6D pose, which just converts the missing error to numerical error, so the accuracy of uni6D is still limited. However, our method calibrate them simultaneously.

% To calibrate depth noise so that reduce the gap between the training and testing dataset, we propose our depth denoise module as ~\ref{fig:depth_denoise_head}. It correct depth based on RoI features with two 3×3 and one 1×1 convolutions to directly regress the depth of visible points. Since XY and depth normal are calculated from depth, we also calibrate them simultaneously, and the correct features are fed into the RT head for the 6D pose estimation..
%

\textbf{Instance-outside Noise Elimination.} 
The most intuitive and efficient choice to filter out the instance-outside noise is directly discarding non-instance regions on the feature map. 
%
However, this feature-level operation can not completely remove the background feature noise because deep features in CNN have a certain receptive field, and the features at the area of the target instance also contains a certain range of surrounding background information.
%
As a result, rather than using the easiest-to-envisage feature-level method, we must filter out the instance-outside noise at the image level.
%
We use Mask R-CNN to obtain the bounding boxes and segmentation results for all instances in the input RGB-D image.
%The most noise out of the bounding box is filtered out by cropping RGB-D patches according to these bounding boxes. And the noise in the non-instance part of the bounding box is further removed by masking cropped patches with segmentation results. 
A majority of instance-outside noise is eliminated by cropping RGB-D patches according to the bounding box. And the rest of instance-outside noise, which remains in the bounding box, is further removed by masking cropped patches with segmentation results.
Corresponding Plain UV, XY, and NRM and PE are also be cropped and masked.
%
% In addition, we also find that dependence of UV encoding is discrepant between detection and 6D pose estimation, UV encoding breaks the convolution translation invariance, which is not friendly to the detection and segmentation, especially when the amount of data is insufficient. 
% %
% For these reasons, we choose the separate network to generate denoised RGB-D patch and corresponding UV encoding as the input of the second step.

%
\textbf{Instance-inside Noise Elimination.} 
As shown in Fig.~\ref{fig:fig1_inside}, the instance-inside noise contains holes and numerical errors in the depth image, both of which affect the performance of the 6D pose estimation task.
%
A widely used method utilizes the classical processing algorithm\Citep{ku2018defense} to fill holes in the raw depth image before regressing the 6D pose. However, the filled pixels in the depth image may still have numerical errors limited by the non-parametric pre-processing method.
%
To handle the instance-inside noise more effectively, we propose a learnable parametric depth denoising module with a noiseless depth estimation task to calibrate the depth information contained in the features. As shown in the second step of Fig.~\ref{fig:framework}, features extracted from RoI Align are fed into our depth denoising module before used to regress the 6D pose.
%
To aid in the convergence of the depth denoising model, we add an auxiliary reconstruction task which regresses the noiseless depth, XY, and NRM simultaneously through a $1\times 1$ convolutional layer.
% 
%The label for the depth estimation task is obtained by calculating the  re-projected depth, XY and NRM from CAD model. 
The supervision labels of the noiseless depth, XY, and NRM are obtained by re-projection from the CAD model.
We use the re-projected depth, XY, and NRM  as supervision labels of denoising module. The noiseless depth and XY are calculated as:
\begin{equation} \label{equ:prj}
  \begin{bmatrix}
    x \\
    y \\
    d 

  \end{bmatrix}
    =
    R^{*} \times
  \begin{bmatrix}
    a  \\
    b  \\
    c 
  \end{bmatrix}
  + T^{*}.
 \end{equation}
For an input visible point $(a,b,c)$ in the CAD model, we apply the ground truth rotation matrix $R^{*}\in SO(3)$ and the translation matrix $T^{*}\in R^3$ to project it to the corresponding position $(x,y,d)$ in camera coordinate system and obtain the re-projected depth and XY.
%
This lightweight depth denoising module can effectively calibrate depth information in features without reducing inference efficiency significantly.
% For inference phase, we firstly correct the feature through denoising module and then feed it into the RT head for the 6D pose estimation.
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.6\textwidth]{figures/fig3.png}
%     \caption{Details of depth denoise module in uni6Dv2.}
%     \label{fig:depth_denoise_head}
% \end{figure}


\subsection{Loss Function}
\label{sec:loss}
The loss function of the entire network consists of the  loss functions of the two steps. The Mask R-CNN is first trained with its original loss~\citep{maskrcnn}.
%Then, we freeze the parameters of the first step and train the network in the second step with the loss of the RT head, abc head, and depth denoising module. 
% 
Then, we freeze the parameters of the first step and train the network in the second step with the RT regression loss, abc regression loss, and the novel depth denoising loss. 
%
The RT regression loss $\mathcal{L}_{rt}$ is deﬁned as:
\begin{equation}
    \mathcal{L}_{rt} = \frac{1}{m}\sum_{x\in\mathcal{O}}||(Rx+T) - (R^*x+T^*)||,
\end{equation}
where $O$ denotes the vertex set of object’s points from the 3D model, $R$ and $T$ are the rotation matrix and the translation vector, $^*$ denotes the ground truth and $m$ is the number of points in $O$. 
%
The abc regression loss is:
\begin{equation}
    \mathcal{L}_{abc} = |a-a^{*}| + |b-b^{*}| + |c-c^{*}|,
\end{equation}
where $(a,b,c)$ are the coordinates of visible points. 
%
The depth denoising loss is:
\begin{equation}
\begin{aligned}
{L}_{depth} = &|d-d^{*}| + |x-x^{*}| + |y-y^{*}|+\\&  |n_x-n_x^{*}| +
|n_y-n_y^{*}| + |n_z-n_z^{*}|,
\end{aligned}
\end{equation}
where $d$ is the depth, $(n_x,n_y,n_z)$ is the coordinate of depth normal calculated from depth, and $(x, y)$ is the visible point's coordinate in camera coordinate system. Finally, the overall loss function of the second step is:
% \begin{equation}\label{equ:loss}
% 	\mathcal{L} = \lambda_0 \cdot \mathcal{L}_{rt} + \lambda_1 \cdot \mathcal{L}_{abc} + \lambda_2 \cdot\mathcal{L}_{depth},
% \end{equation}
\begin{equation}\label{equ:loss}
	\mathcal{L} = \lambda_0  \mathcal{L}_{rt} + \lambda_1  \mathcal{L}_{abc} + \lambda_2 \mathcal{L}_{depth},
\end{equation}
where $\lambda_0$, $\lambda_1$ and $\lambda_2$ are the weights for each loss.


==> sec/4exp_overview_bk.tex <==
\section{EXPERIMENTS}
\label{others}
\subsection{Benchmark Datasets}
\label{sec:datasets}
We compare the proposed method with others on  three benchmark datasets. 

\textbf{YCB-Video}\Citep{calli2015ycb} contains 92 RGB-D videos with 21 YCB objects, which has depth noise and occlusions. Following previous work\Citep{posecnn,pvn3d,densefusion,uni6d}, we add synthetic images for training and the synthetic ratio is 83.17$\%$. We also apply the hole completion algorithm used in\Citep{pvn3d,uni6d} to improve depth images.

\textbf{LineMOD}\Citep{hinterstoisser2011multimodal} contains 13 videos of 13 low-textured objects. Following previous works\Citep{peng2019pvnet,posecnn,pvn3d,uni6d}, we also add synthetic images for training and the synthetic ratio is 99.71$\%$.

\textbf{Occlusion LineMOD}\Citep{brachmann2014learning} is selected from the LineMOD dataset, which has heavily occluded objects, making the scenes more challenging.

\subsection{Evaluation Metrics}

We use the average distance metrics ADD and ADD-S to evaluate our method, following\Citep{posecnn,densefusion,ffb6d,uni6d}. The ADD metric\Citep{hinterstoisser2012model} is calculated as follows:
\begin{equation}
    \begin{split}
        \textrm{ADD} = \frac{1}{m}\sum_{x\in\mathcal{O}}||(Rx+T) - (R^*x+T^*)||,
    \end{split}
\end{equation}
where $m$ is the total vertex number, $x$ indicates any vertex of the 3D model $\mathcal{O}$,  $[R, T]$ and $[R^*, T^*]$ are predicted pose and ground truth pose respectively. The ADD-S is similar to ADD, but is used to measure the performance of symmetric objects, which is based on the closest point distance: 
%
\begin{equation}
    \begin{split}
        \textrm{ADD-S} = \frac{1}{m}\sum_{x_{1}\in\mathcal{O}}\min_{x_{2}\in\mathcal{O}}||(Rx_{1}+T) - (R^*x_{2}+T^*)||.
    \end{split}
\end{equation}
%
For convenience, the ADD(S) metric is introduced as follows:
\begin{eqnarray}
\textrm{ADD(S)} =
\begin{cases}
\textrm{ADD}   & \mathcal{O}~is~asymmetric\\
\textrm{ADD-S} & \mathcal{O}~is~symmetric 
\end{cases}
\end{eqnarray}
where $\mathcal{O}$ is the CAD model.

For YCB-Video dataset, the area under the accuracy-threshold curve obtained by varying the distance threshold with a maximum threshold of 0.1 meters (AUC ADD-S or AUC ADD(S)) is reported, following previous works \Citep{posecnn,densefusion,pvn3d,ffb6d}. 
%The ADD(S) means measure asymmetric object by ADD and symmetric object by ADD-S.
For LineMOD and Occlusion LineMOD datasets, the accuracy of distance less than 10\% of the objects' diameter (ACC ADD(S)-0.1d) is reported, following previous works \Citep{peng2019pvnet,ffb6d}

% we follow\Citep{posecnn,densefusion,pvn3d,ffb6d} to compute the ADD-S and ADD(S) under the accuracy-threshold curve obtained by varying the distance threshold with maximum threshold 0.1 meter (ADD-0.1). 



\begin{table*}[ht]
\begin{center}
\caption{Evaluation results on the YCB-Video dataset. Symmetric objects are denoted in bold.}
\vspace{.15in}
\label{tab:ycb}
\resizebox{0.99\linewidth}{!}{
% \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c}
\begin{tabular}{lcccccccccccc}
    \toprule
 & \multicolumn{2}{c}{PoseCNN\Citep{posecnn}}  & \multicolumn{2}{c}{DenseFusion\Citep{densefusion}} & \multicolumn{2}{c}{PVN3D\Citep{pvn3d}} & \multicolumn{2}{c}{FFB6D\Citep{ffb6d}} & \multicolumn{2}{c}{Uni6D\Citep{uni6d}} & \multicolumn{2}{c}{Ours} \\ 
    \midrule
 Object & \small{ADD-S} & \small{ADD(S)} & \small{ADD-S} & \small{\small{ADD(S)}} & \small{ADD-S} & \small{ADD(S)} & \small{ADD-S} & \small{ADD(S)} & \small{ADD-S} &\small{ADD(S)} & \small{ADD-S} &\small{ADD(S)}\\ \midrule
        002\_master\_chef\_can & 83.9 & 50.2 & 95.3 & 70.7 & 96 & 80.5 & 96.3 & 80.6 & 95.4 & 70.2 & 96.0 & 74.2  \\
        003\_cracker\_box & 76.9 & 53.1 & 92.5 & 86.9 & 96.1 & 94.8 & 96.3 & 94.6 & 91.8 & 85.2 & 96.0 & 94.2 \\ 
        004\_sugar\_box & 84.2 & 68.4 & 95.1 & 90.8 & 97.4 & 96.3 & 97.6 & 96.6 & 96.4 & 94.5 & 97.6 & 96.6 \\ 
        005\_tomato\_soup\_can & 81.0 & 66.2 & 93.8 & 8.47 & 96.2 & 88.5 & 95.6 & 89.6 & 95.8 & 85.4 & 96.1 & 86.6 \\
        006\_mustard\_bottle & 90.4 & 81.0 & 95.8 & 90.9 & 97.5 & 96.2 & 97.8 & 97.0 & 95.4 & 91.7 & 97.8 & 96.7 \\   % drop
        007\_tuna\_fish\_can & 88.0 & 70.7 & 95.7 & 79.6 & 96.0 & 89.3 & 96.8 & 88.9 & 95.2 & 79.0 & 96.3 & 76.0 \\ 
        008\_pudding\_box & 79.1 & 62.7 & 94.3 & 89.3 & 97.1 & 95.7 & 97.1 & 94.6 & 94.1 & 89.8 & 96.6 & 94.7 \\ 
        009\_gelatin\_box & 87.2 & 75.2 & 97.2 & 95.8 & 97.7 & 96.1 & 98.1 & 96.9 & 97.4 & 96.2 & 98.0 & 97.0 \\  % drop
        010\_potted\_meat\_can & 78.5 & 59.5 & 89.3 & 79.6 & 93.3 & 88.6 & 94.7 & 88.1 & 93.0 & 89.6 & 95.7 & 91.9 \\ 
        011\_banana & 86.0 & 72.3 & 90.0 & 76.7 & 96.6 & 93.7 & 97.2 & 94.9 & 96.4 & 93.0 & 98.0 & 96.9 \\ % drop
        019\_pitcher\_base & 77.0 & 53.3 & 93.6 & 87.1 & 97.4 & 96.5 & 97.6 & 96.9 & 96.2 & 94.2 & 97.5 & 96.9 \\  % drop
        021\_bleach\_cleanser & 71.6 & 50.3 & 94.4 & 87.5 & 96.0 & 93.2 & 96.8 & 94.8 & 95.2 & 91.1 & 97.0 & 95.3 \\  % drop
        \textbf{024\_bowl} & 69.6 & 69.6 & 86.0 & 86.0 & 90.2 & 90.2 & 96.3 & 96.3 & 95.5 & 95.5 & 96.8 & 96.8 \\ 
        025\_mug & 78.2 & 58.5 & 95.3 & 83.8 & 97.6 & 95.4 & 97.3 & 94.2 & 96.6 & 93.0 & 97.7 & 96.3 \\  % drop
        035\_power\_drill & 72.7 & 55.3 & 92.1 & 83.7 & 96.7 & 95.1 & 97.2 & 95.9 & 94.7 & 91.1 & 97.6 & 96.8 \\  % drop
        \textbf{036\_wood\_block} & 64.3 & 64.3 & 89.5 & 89.5 & 90.4 & 90.4 & 92.6 & 92.6 & 94.3 & 94.3 & 96.1 & 96.1 \\ 
        037\_scissors & 56.9 & 35.8 & 90.1 & 77.4 & 96.7 & 92.7 & 97.7 & 95.7 & 87.6 & 79.6 & 95.0 & 90.3 \\  % drop
        040\_large\_marker & 71.7 & 58.3 & 95.1 & 89.1 & 96.7 & 91.8 & 96.6 & 89.1 & 96.7 & 92.8 & 97.0 & 93.1 \\
        \textbf{051\_large\_clamp} & 50.2 & 50.2 & 71.5 & 71.5 & 93.6 & 93.6 & 96.8 & 96.8 & 95.9 & 95.9 & 97.0 & 97.0 \\  % drop
        \textbf{052\_extra\_large\_clamp} & 44.1 & 44.1 & 70.2 & 70.2 & 88.4 & 88.4 & 96.0 & 96.0 & 95.8 & 95.8 & 96.5 & 96.5 \\  % drop
        \textbf{061\_foam\_brick} & 88.0 & 88.0 & 92.2 & 92.2 & 96.8 & 96.8 & 97.3 & 97.3 & 96.1 & 96.1 & 97.4 & 97.4 \\ % drop \midrule[1pt]
        \midrule
        Avg & 75.8 & 59.9 & 91.2 & 82.9 & 95.5 & 91.8 & 96.6 & 92.7 & 95.2 & 88.8 & 96.8 & 91.5 \\   \bottomrule
\end{tabular}}
\end{center}                        
\end{table*}

\begin{table*}[ht]
\begin{center}
\caption{Evaluation results (ACC \small{ADD(S)}-0.1d) on the LineMOD dataset. Symmetric objects are denoted in bold.}

\label{tab:LineMOD-ADD}
\resizebox{1\linewidth}{!}{
% \begin{tabular}{l|c|c|c|c|c|c}
\begin{tabular}{lcccccc}
    \toprule
 & PoseCNN\Citep{posecnn} & DenseFusion\Citep{densefusion} & PVN3D\Citep{pvn3d} & FFB6D\Citep{ffb6d} & Uni6D\Citep{uni6d} & Ours \\
    \midrule
      ape & 77.0   & 92.3 & 97.3 & 98.4 & 93.71 & 95.71 \\
      benchvise & 97.5  & 93.2 &  99.7 & 100.0 & 99.81 & 99.90 \\
      camera & 93.5 & 94.4  & 99.6 & 99.9 & 95.98 & 95.78\\
      can & 96.5  & 93.1 & 99.5 & 99.8 & 99.02 & 96.01\\
      cat & 82.1  & 96.5 & 99.8 & 99.9 & 	98.10 & 99.20\\
      driller & 95.0  & 87.0 & 99.8 & 100.0 & 99.11 & 99.21\\
      duck & 77.7  & 92.3 & 97.7 & 98.4 & 89.95 & 92.11\\
      \textbf{eggbox} & 97.1  & 99.8 & 99.8 & 100.0 & 100.00 & 100.00 \\
      \textbf{glue} & 99.4  & 100.0 & 100.0 & 100.0 & 99.23 & 99.61\\ 
      holepuncher & 52.8 & 92.1 &  99.9 & 99.8 & 90.20 & 92.01\\
      iron & 98.3  & 97.0  & 99.7 & 99.9 & 99.49 & 97.96\\
      lamp & 97.5 & 95.3  & 99.8 & 99.9 & 99.42 & 98.46\\
      phone & 87.7  & 92.8  & 99.5 & 99.7 &97.41 & 97.69\\
      \hline
      Avg & 88.6 & 94.3  & 99.4 & 99.7 & 97.03  & 97.20\\   \bottomrule
\end{tabular}}
\end{center}                        
\end{table*}

\begin{table*}[t]
\begin{center}
\caption{Evaluation results (ACC \small{ADD(S)}-0.1d) on the Occlusion LineMOD dataset. Symmetric objects are denoted in bold.}
\vspace{.15in}
\label{tab:ocLineMOD-ACC}
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{lccccc}
    \toprule
 Method & PoseCNN\Citep{posecnn}   & PVN3D\Citep{pvn3d} & FFB6D\Citep{ffb6d} & Uni6D\Citep{uni6d} & Ours \\
    \midrule
      ape & 9.6  &  33.9 & 47.2 & 32.99 & 44.26 \\
      can & 45.2  & 88.6 & 85.2 & 51.04 & 53.33\\
      cat & 0.9  & 39.1 & 45.7 & 4.56 & 16.70\\
      driller & 41.4 & 78.4 & 81.4 & 58.40 & 63.02\\
      duck & 19.6  & 41.9 & 53.9 & 34.80 & 38.09\\
      \textbf{eggbox} & 22.0  & 80.9 & 70.2 & 1.73 & 4.60  \\
      \textbf{glue} & 38.5   & 68.1 & 60.1 & 30.16 & 40.27 \\ 
      holepuncher & 22.1  & 74.7 & 85.9 & 32.07 & 50.93\\
       \hline
        Avg & 24.9  & 63.2 & 66.2 & 30.71 & 40.15 \\ \bottomrule
\end{tabular}}
\end{center}                        
\end{table*}

% \subsection{Comparison with Other Methods}
% We compare our method with others on YCB-Video, LineMOD, and Occlusion LineMOD datasets. The results of YCB-Video dataset are presented in main paper and the results of LineMOD and Occlusion LineMOD are shown in our Appendix.
\subsection{Comparison with Other Methods}
We compare our method with others on YCB-Video, LineMOD, and Occlusion LineMOD datasets.

\subsubsection{Evaluation on YCB-Video Dataset}
We present the category-level results of the proposed Uni6Dv2 on YCB-Video dataset in Table~\ref{tab:ycb}. Compared with other methods, our approach advances state-of-the-art results by 0.2$\%$ on the ADD-S metric and achieves 91.5$\%$ on the ADD(S) metric. It is worth emphasizing that Uni6Dv2 comprehensively exceeds Uni6D, especially on objects with fewer pixels.
For example, "037\_scissors" of Uni6Dv2 achieves 7.36$\%$ improvement on the ADD-S metric and 9.72$\%$ on the ADD(S).

\subsubsection{Evaluation on LineMOD Dataset}
Experimental results of LineMOD dataset are reported in Table~\ref{tab:LineMOD-ADD}, our approach achieves 97.20\% ACC ADD(S)-0.1d. Compared with the original Uni6D, it improves the performance in "ape", "benchvise", "cat", "driller", "duck", "glue", "holepuncher" and "phone". Because the LineMOD dataset has less depth noise and occlusion than the YCB-Video dataset, our two-step denoising method make improvement slightly.

\subsubsection{Evaluation on Occlusion LineMOD Dataset}
We train our model on the LineMOD dataset and evaluate it on the Occlusion LineMOD dataset to obtain the performance on occlusion scene. Experimental results of Occlusion LineMOD are reported in Table~\ref{tab:ocLineMOD-ACC}. Compared with Uni6D, our method obtains 9.44\% improvement on the ACC ADDS-0.1d metric, and the ACC ADDS-0.1d of all categories have been improved.

\subsection{Time Efficiency}
We compare the inference speed of our method with PoseCNN\Citep{posecnn}, DenseFusion\Citep{densefusion}, PVN3D\Citep{pvn3d}, FFB6D\Citep{ffb6d}, and Uni6D\Citep{uni6d} in Table~\ref{tab:time} and Fig.~\ref{fig:efficieny}.
Our method achieves 21.27 FPS which is $6\times$ faster than FFB6D (SOTA of keypoint-base methods). Compared with Uni6D (SOTA of RoI-based methods), our methods only sacrifices 17\% efficiency to achieve significant gains especially without real training data in Table~\ref{tab:lack-real} (\textbf{+20.11\%} ADD-S and \textbf{+29.48\%} ADD(S)). 
%our method still maintains time efficiency than the method with two heterogeneous backbones, which is $6\times$ faster than FFB6D, and $11\times$ than PVN3D.
%
More specifically, the first and second steps of our method take \SI{35}{ms} and \SI{12}{ms}, the extra computation is mainly added on the backbone in the second step, so it is a little slower than Uni6D.

\begin{table}[htb]
   \centering
     \caption{Time cost and frames per second (FPS) on YCB-Video Dataset.
     %The results of PoseCNN and DenseFusion come from their papers\Citep{densefusion}, which does not specify the type of device used.
     } 
     \vspace{.15in}
     \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{ccccc}
    \toprule
        %  PoseCNN+ICP\Citep{posecnn} &  DenseFusion\Citep{densefusion} & Our  Uni6D \\
        Method & Network/ms & Post-process/ms & All/ms & FPS \\
        \midrule
        PoseCNN\Citep{posecnn} & 200 & \textbf{0} & 200 & 5 \\
        DenseFusion\Citep{densefusion} & 50 & 10 & 60 &  16.67\\
        PVN3D\Citep{pvn3d} & 110 & 420 & 530 & 1.89\\
        FFB6D\Citep{ffb6d} & \textbf{20} & 260 & 280 & 3.57 \\
        Uni6D\Citep{uni6d} & 39 & \textbf{0} & \textbf{39} & \textbf{25.64} \\
        Ours & 47 & \textbf{0} & 47 & 21.27 \\
    \bottomrule
    \end{tabular}}
    \label{tab:time} 
\end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/fig_time_acc.png}
    \caption{Comparison of effectiveness and efficiency.}
    \label{fig:efficieny}
\end{figure}

\makeatletter
\newcommand\figcaption{\def\@captype{figure}\caption}
\newcommand\tabcaption{\def\@captype{table}\caption}
\makeatother
%\fi
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1.0\textwidth]{figures/fig_qualitative vis.png}
%     \caption{Time efficiency and accuracy}
%     \label{fig:efficieny}
% \end{figure*}
